Few-shot Adaptation Works with UnpredicTable Data

Prior work on language models (LMs) shows that training on a large number of diverse tasks improves few-shot learning (FSL) performance on new tasks. We take this to the extreme, automatically extracting 413,299 tasks from internet tables - orders of magnitude more than the next-largest public datasets. Finetuning on the resulting dataset leads to improved FSL performance on Natural Language Processing (NLP) tasks, but not proportionally to dataset scale. In fact, we find that narrow subsets of our dataset sometimes outperform more diverse datasets. For example, finetuning on software documentation from support.google.com raises FSL performance by a mean of +7.5% on 52 downstream tasks, which beats training on 40 human-curated NLP datasets (+6.7%). Finetuning on various narrow datasets leads to similar broad improvements across test tasks, suggesting that the gains are not from domain adaptation but adapting to FSL in general. We do not observe clear patterns between the datasets that lead to FSL gains, leaving open questions about why certain data helps with FSL.

==> tables/annotations_example_tasks_classes.tex <==
\newpage
\begin{figure*}[ht!]
\begin{tabular}[ht!]{|c|p{0.9\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Criteria and Examples of Class 0 (low rating) Tasks}}} \\
\hline
Criteria & \begin{itemize}
    \item The input-output mapping appears nonsensical and/or arbitrary.
    \item The task is not in English.
    \item Would never be useful in any realistic setting / practicing this task does not build any generally-useful skills.
    \item Tests highly obscure knowledge that is not correlated with the input text (highly context-dependent knowledge, entertainment trivia on fan sites, product specifications, …)
    \item You would not even be able to tell if all output labels have been shuffled.
\end{itemize} \\
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 1}} \\
\hline
input & [Artist] Zebra Stripes [Title] \\
output & Intro '66 \\ [5pt]
\hdashline
input & [Artist] the High Spirits [Title] \\
output & It's Alright With Me \\ [5pt]
\hdashline
input & [Artist] Chob [Title] \\
output & We're Pretty Quick \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 2}} \\
\hline
input & [Feature] Bullet support in paragraph styles [Issue\#] 102 [Status] \\
output & DONE \\ [5pt]
\hdashline
input & [Feature] Hyphenation improvements [Comments] assigned to cezaryece [Issue\#] 417 [Status] \\
output & IN PROGRESS \\ [5pt]
\hdashline
input & [Feature] Text refinements [Comments] assigned to cezaryece [Issue\#] 415 [Status] \\
output & IN PROGRESS \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 3}} \\
\hline
input & [Bowl Height] Product Weight (lb.) [Comfort Height] 103 lb [Elongated] 90-Day [Bowl Shape] \\
output & Returnable \\ [5pt]
\hdashline
input & [Bowl Height] Rough In Size [Comfort Height] 12 [Elongated] No Additional Features [Bowl Shape] \\
output & Toilet Features \\ [5pt]
\hdashline
input & [Bowl Height] Toilet Included Components [Comfort Height] Seat [Elongated] Left Side [Bowl Shape] \\
output & Trip Lever Location \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 4}} \\
\hline
input & [Language] Norwegian [Name] Det tapre lokomotivet [Meaning] \\
output & The Brave Engine \\ [5pt]
\hdashline
input & [Language] Italian [Name] La locomotiva coraggiosa [Meaning] \\
output & The Courageous Engine \\ [5pt]
\hdashline
input & [Language] Japanese [Name] \begin{CJK}{UTF8}{min}ゆうかんなきかんしゃ\end{CJK} [Meaning] \\
output & Brave Engine \\ [5pt]
\hline
\end{tabular}
\caption{Criteria and Examples of Class 0 (low rating) Tasks.}
\label{tab:annotations_example_tasks_class0}
\end{figure*}

\newpage
\begin{figure*}[ht!]
\begin{tabular}[ht!]{|c|p{0.9\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Criteria and Examples of Class 1 (medium rating) Tasks}}} \\
\hline
Criteria & \begin{itemize}
    \item This class is a catch-all for tasks that are neither squarely Class 0 nor Class 2.
    \item The task is quite interesting, but its current form contains flaws that make it confusing or lacks enough context to do a good job of the task.
    \item You could narrow the space of possible options and guess the right answer with better-than-random accuracy (especially with the help of multiple-choice options).
    \item The task makes sense but is trivial or not interesting enough to be Class 2. For example, the output is just a copy of the input.
\end{itemize} \\
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 1}} \\
\hline
input & [Skill Name] Accuracy [Japanese] \begin{CJK}{UTF8}{min}白刃一閃\end{CJK} [Requirements] Defeat an enemy officer with a chain above a certain length. [Effects] \\
output & Increases chance of inflicting a critical hit. \\ [5pt]
\hdashline
input & [Skill Name] Quick Learner [Japanese] \begin{CJK}{UTF8}{min}守破離心得\end{CJK} [Requirements] Defeat an enemy officer that is afflicted with a status ailment. [Effects] \\
output & Adds a bonus to the amount of experience earned. \\ [5pt]
\hdashline
input & [Skill Name] Fortune Hunter [Japanese] \begin{CJK}{UTF8}{min}慶雲招来\end{CJK} [Requirements] Defeat an enemy officer with a KO count above a certain level. [Effects] \\
output & Increases character's luck. \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 2}} \\
\hline
input & [0] No Implant Attempt [Description] \\
output & Subjects who did not undergo an implant attempt of a CRT-P or CRT-D device and were not randomized \\ [5pt]
\hdashline
input & [0] Unsuccessful Implants [Description] \\
output & Subjects who underwent an implant attempt of a CRT-P or CRT-D device but were not successfully implanted \\ [5pt]
\hdashline
input & [0] CRT-P: Biventricular Pacing Arm [Description] \\
output & Subjects who were implanted with a CRT-P device and randomized to receive biventricular pacing \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 3}} \\
\hline
input & [Categories] Campus Safety [Comments] \\
output & We have security guards all across campus 24/7. I feel extremely safe here, even at night. \\ [5pt]
\hdashline
input & [Categories] Great for these types of students [Comments] \\
output & If you love the arts, then you will love Southeastern's Communication and Music departments. We always put on spectacular performances. \\ [5pt]
\hdashline
input & [Categories] Bang for the buck [Comments] \\
output & One thing about being at a private collage is that it can be pretty expensive. It does take a lot of work searching for scholarships and other aid to continue my education. \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 4}} \\
\hline
input & [Option] --emailFrom [Default] Address of build master [Description] \\
output & Becomes the sender of the emails sent from the aggregator. \\ [5pt]
\hdashline
input & [Option] --mockEmailTo [Default] no value [Description] \\
output & Becomes the receiver of the mock-emails sent from the aggregator. If not set, no mock emails are sent. \\ [5pt]
\hdashline
input & [Option] --logLevel [Value] DEBUG INFO WARNING ERROR [Default] INFO [Description] \\
output & Controls the verbosity of the console trace output. Defaults to global b3 settings. \\ [5pt]
\hline
\end{tabular}
\caption{Criteria and Examples of Class 1 (medium rating) Tasks.}
\label{tab:annotations_example_tasks_class1}
\end{figure*}

\newpage
\begin{figure*}[ht!]
\begin{tabular}[ht!]{|c|p{0.9\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Criteria and Examples of Class 2 (high rating) Tasks}}} \\
\hline
Criteria & \begin{itemize}
    \item The task is well-posed with enough context that an expert could give a reasonably correct answer most of the time.
    \item Demonstrates a skill that is definitely useful for real-world tasks i.e. might be tested in an exam or competency test, or part of a job.
    \item Resembles the type of skill that is tested in typical NLP datasets. See “Examples from real NLP datasets” below.
\end{itemize} \\
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 1}} \\
\hline
input & [0] Decision-making is a very vital part in our lives. This is [Correction] of [Error] \\
output & in \\ [5pt]
\hdashline
input & [0] the present. That is not possible to reverse the wrong [Correction] it [Error] \\
output & That \\ [5pt]
\hdashline
input & [0] tomorrow will be a result of the decisions we took in [Correction] the [Error] \\
output & a \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 2}} \\
\hline
input & [Definition] Searches meta data for specified text. Meta data includes the item’s title, description, details, comments, and tags. Returns only those items with the exact text specified as the Keyword. [Affects] All items [Filter] \\
output & Keyword \\ [5pt]
\hdashline
input & [Definition] Displays only works of art created in a specific medium, such as sculpture and architecture. [Affects] Works of Art [Filter] \\
output & Medium \\ [5pt]
\hdashline
input & [Definition] Displays only works of art created by a specific artist. Artist name can be entered in First Name-Last Name order or Last Name-First Name order. List autocompletes. [Affects] Works of Art [Filter] \\
output & Artist \\ [5pt]
\hline
\multicolumn{2}{|c|}{Table is contined on the next page.} \\
\hline
\end{tabular}
\end{figure*}

\newpage
\begin{figure*}[ht!]
\begin{tabular}[ht!]{|c|p{0.9\linewidth}|}
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Continuation of Criteria and Examples of Class 2 (high rating) Tasks}}} \\
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 3}} \\
\hline
input &  [Author] sourtaste Prince George, VA (1 review) August 17, 2011 [Content] I wanted to report that this was a good experience, but I can not. Last fall my dogwood trees were so late coming we had snow on the ground when I received them. Was supposed to receive notification that they had been shipped. I did not receive any notice. There were no instructions in the clear plastic bag with my trees. My trees never sprouted this season so I notified the service email address. The same address I used when questioning where my shipment was. It has been 23 days and 3 emails and no response at all. What about the guarantee? I like to help these types of organizations when I get the chance. Just wish there hadn't been false advertisement with the satisfaction guarantee. They were quite prompt in taking my money months before shipping the product. [Rating] \\
output & Negative \\ [5pt]
\hdashline
input & [Author] heatherMO Mount Vernon, MO (1 review) April 29, 2011 [Content] My son came home from school with a pine tree he recieved (donated by a local company who purchased it from freetreesandplants.com). It rained quite heavily for the following 4 days, so i placed the tree (still in it's original bag) in the refrigerator as suggested. When the sun finally came out again, we got the tree out of the fridge, and it still looked great. We followed the directions included and then planted it in the ground...and it is doing great! I am extreamly pleased with our tree, and found it quite inspiring that there are still people out there willing to do good and help others in the process And my son sure is proud of his new addition to our landscaping! : ) [Rating] \\
output & Positive \\ [5pt]
\hdashline
input & [Author] earlbishop Independence, MO (1 review) May 15, 2009 [Content] Nothing but positives about my experience with these people. They answered my e-mails and/or phone calls promptly and courteously. My order was shipped at the time they promised and arrived in good shape. The plants were healthy when I put them in the ground. Waiting for survival rate because an hour after planting we experienced 4-6 inch rainfall. The plants looked good before they were inundated. I will definitely order again and refer friends to the site. [Rating] \\
output & Positive \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 4}} \\
\hline
input & [Name] url [Description] the URL of the data repository [mandatory?] no [Type] \\
output & string \\ [5pt]
\hdashline
input & [Name] success [Description] true if the page contains any records, otherwise false [mandatory?] no [Type] \\
output & boolean \\ [5pt]
\hdashline
input & [Name] results [Description] the total number of records matching the request [mandatory?] no [Type] \\
output & integer \\ [5pt]
\hline
\multicolumn{2}{|c|}{\textbf{Example Task 5}} \\
\hline
input & [Question] carry [Answer] \\
output & carried \\ [5pt]
\hdashline
input & [Question] marry [Answer] \\
output & married \\ [5pt]
\hdashline
input & [Question] bury [Answer] \\
output & buried \\ [5pt]
\hline
\end{tabular}
\caption{Criteria and Examples of Class 2 (high rating) Tasks.}
\label{tab:annotations_example_tasks_class2}
\end{figure*}

==> tables/predictable_examples_example_tasks.tex <==
\clearpage
\begin{center}
\begingroup
\renewcommand{\arraystretch}{1.2}
\begin{tabular}[h]{|l|l|}
\hline
\multicolumn{2}{|c|}{\textbf{\textit{Example task}}} \\
\hline

\multicolumn{2}{|c|}{\textbf{Task 1}} \\
\hline
INPUT &  [Question] The parotid glands are located: [Answer] \\
OUTPUT & cheeck  \\
\hdashline
INPUT & [Question] The roof of the mouth is called the: [Answer] \\
OUTPUT & hard palte \\ [5pt]
\hdashline
INPUT &  [Question] The bone that forms the posterior portion of the skull is the [Answer] \\
OUTPUT &  occipital bone \\ [5pt]
\hline

\multicolumn{2}{|c|}{\textbf{Task 2}} \\
\hline
INPUT &  [Question] The parotid glands are located: [Answer] \\
OUTPUT & cheeck  \\
\hdashline
INPUT & [Question] The roof of the mouth is called the: [Answer] \\
OUTPUT & hard palte \\ [5pt]
\hdashline
INPUT &  [Question] The bone that forms the posterior portion of the skull is the [Answer] \\
OUTPUT &  occipital bone \\ [5pt]
\hline

\multicolumn{2}{|c|}{\textbf{Task 3}} \\
\hline
INPUT &  [Question] The parotid glands are located: [Answer] \\
OUTPUT & cheeck  \\
\hdashline
INPUT & [Question] The roof of the mouth is called the: [Answer] \\
OUTPUT & hard palte \\ [5pt]
\hdashline
INPUT &  [Question] The bone that forms the posterior portion of the skull is the [Answer] \\
OUTPUT &  occipital bone \\ [5pt]
\hline

\multicolumn{2}{|c|}{\textbf{Task 4}} \\
\hline
INPUT: &  [Question] The parotid glands are located: [Answer] \\
OUTPUT: & cheeck  \\
\hdashline
INPUT: & [Question] The roof of the mouth is called the: [Answer] \\
OUTPUT: & hard palte \\ [5pt]
\hdashline
INPUT: &  [Question] The bone that forms the posterior portion of the skull is the [Answer] \\
OUTPUT: &  occipital bone \\ [5pt]
\hline
%\caption{Examples few shot data from example Task}
%\label{tab:example_summaries}
\end{tabular}
\endgroup
\end{center}
\clearpage

